DeepStrike: Remotely-Guided Fault Injection Attacks on DNN Accelerator in Cloud-FPGA

As Field-programmable gate arrays (FPGAs) are widely adopted in clouds to accelerate Deep Neural Networks (DNN), such virtualization environments have posed many new security issues. This work investigates the integrity of DNN FPGA accelerators in clouds. It proposes DeepStrike, a remotely-guided attack based on power glitching fault injections targeting DNN execution. We characterize the vulnerabilities of different DNN layers against fault injections on FPGAs and leverage time-to-digital converter (TDC) sensors to precisely control the timing of fault injections. Experimental results show that our proposed attack can successfully disrupt the FPGA DSP kernel and misclassify the target victim DNN application.

==> Achieve/case_study.tex <==
\section{Experimental setup and validation results}



\subsection{Multi-tenant FPGA power glitch \TDCattack}\label{sec:attacking_scheduler}
A controllable DNN power attack means that the attacker can activate the power-plundering circuit at a specific moment, such as a particular computing layer, and place a certain number of attacks during this period. 
Our threat model assumes the attacker does not have any knowledge about the model’s parameters. 
Thus, a fine-tuning attack on the specific weight or pixel computing procedure is impossible. 
However, the power leakage measurement through the TDC-based delay-sensor can provide enough information to the attacker so that s/he can place a specific number of attacks on the target computing period. 
To implement this attacking scheme, we design a power glitch attacking scheduler to guide the attack. 
Figure \ref{Fig:ATK_scheduler} shows the architecture of the attacking scheduler, including a TDC-based delay-sensor, malicious circuits (power plundering circuits or high-load applications), a signal RAM, an attack controller, and an attacking scheme file. 
As we mentioned in section \ref{sec:atk_step}, the TDC-based delay-sensor in the preparing step can trace the target DNN runtime power fluctuation. 
While we gather those leakages, this TDC-based delay-sensor can be used to detect the starting point of the target DNN application execution. 
The sensor triggers the attacking controller, and the power-plundering circuit activation signal is designed by the attacker and stored in the signal RAM. 
This file includes three critical parameters: \textit{attack delay}, \textit{attack period}, and \textit{the number of attacks}. \\
The \textit{attack delay} can target a specific DNN computing layer. The \textit{attack period} provides constraint to attack placement. And the \textit{number of attacks} determines how many attacks happen in an attack period. 
The most high-light part is that the attacker can load her/his attack scheme to a signal RAM in runtime. 
This feature can allow the attacker to place different attack schemes and achieve an efficient prediction accuracy reduction in the target DNN.

%%\vspace{-0.5em}
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\linewidth]{FIG/FIG_TDC_Guide.pdf}
    \caption{TDC-based delay-sensor DNN \TDCattack architecture. \textcolor{red}{remember to add extra space if you use pre-defined abbreviations. Also, is it delay-sensor, or voltage sensor, sync the words in this paper.}}
    \label{Fig:ATK_scheduler}
    %%\vspace{-1.5em}
\end{figure}

%\subsection{DPU+DNNDK framework: implementing different DNN with Visit AI Model Zoo} 
%\noindent Xilinx provides a DPU+DNNDK framework, which can generate a specific deep learning acceleration unit for different devices. DNNDK is a software-level DPU controller embedded with popular DNN frameworks, such as Tensorflow, Pytorch to create a systematic DNN builder. Briefly introduce the DPU+DNNDK framework in this section, and mention that our Ex.1 convolutional kernel is based on DPU structure. 

\subsection{Case study}\label{sec:case_study}


% %%\vspace{-0.5em}
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\linewidth]{FIG/FIG_MNIST_Case_study.pdf}
    \caption{Case study result: apply DeepStrike on MNIST application.}
    \label{Fig:MNIST_Result}
    % %%\vspace{-1.5em}
\end{figure}
PYNQ is an open-source project that integrates the Linux system with the Xilinx FPGA to build a platform. 
It is used by developers to efficiently deploy hardware-software co-designed applications on the FPGA and control it through high-level languages, such as python. 
Multiple Xilinx devices such as Zynq-7000 and ultrascale+ FPGA families can support this platform. 
In our threat model, the hypervisor in the virtualized cloud-FPGA will compile and combine the attacker’s malicious circuits with the victim tenant’s DNN application, and generate and deploy them on one FPGA device. 
Based on this scenario, we apply Pynq-z1 to build a prototype of the cloud-FPGA. 
The benign user remotely  builds up a DNN application by utilizing the pynq library, and the attacker connects to this prototype cloud-FPGA from the UART serial port. 
We manually combine their hardware applications into one bitstream, like most FPGA virtualization articles claim \cite{zha2020virtualizing}. 
We also isolate those two applications without I/O bus, BRAM, or clock source sharing. 
The test DNN application refers to the LeNet architecture \cite{lecun2015lenet,Wang_FCCM18} and we train the model with the MNIST dataset \cite{MNIST_data}. 
The parameters of this model are 8-bits for the fixed-point value, 3-bits for integers, and the rest for mantissa representation. 
For this dataset, it includes $60,000$ training samples and $10,000$ testing samples. And our model infers that the testing set can achieve an accuracy of $96.17\%$ without any attacks in the FPGA. 
The architecture of LeNet is shown in figure \ref{Fig:MNIST_Result}, where “Conv” is the convolution acceleration kernel, which is the “filter” for images. 
“Pool” represents the pooling layer for downsampling usage. 
“FC” is the fully connection layer, which compiles the inputs from previous layers and generates a final prediction for each target class. 
Here we need to highlight that as we use the unsign fixed-point quantization method the activation function we use in this case study is the hyperbolic tangent (tanh).
We target each layer separately and apply several attacks while the corresponding acceleration kernel is executing.
We observe the inference accuracy, and the result in figure \ref{Fig:MNIST_Result} shows that our proposed scheme can achieve a maximum $14\%$ accuracy reduction when we apply $4500$ times attacks on the convolution layer 2. 
Each attack triggers the power plundering circuits for $10 ns$, and the power plundering circuit consumes $15.03\%$ logic slices. 
The resistance of power glitch attack in each layer depends on the execution time, the layer’s type, and the layer’s location. 
Comparing layer 1 and 2, both of them are convolution layers. However, layer 2 has a longer execution time, which means we can apply more attacks in layer 2, and it can achieve more accuracy reduction. 
Layer 4 has the longest execution time. It is a fully connection layer, unlike the convolution layer, which only adds $k \times k$ numbers multiplication results to generate one pixel in a feature map. The fully connection layer adds all multiplication results from input together. 
Suppose the attack happens while the accelerator is computing. As we show in section \ref{sec:DSP}, the attack may generate random faults or duplication faults, and the correct product will appear in the next clock. 
In this scenario, more serial summation will mitigate the impaction of junk data. 
That is why FC 1 cannot achieve too much reduction as Conv 2 does while applying the same number of attacks. 
We also provide the result of non-TDC guiding attacks with figure \ref{Fig:MNIST_Result} as our baseline. 
We can conclude that our proposed TDC guiding attack method is more efficient than the blind attack while applying the same attack intensity. 




==> Achieve/experiment_ideas.tex <==
1. DSP fault type analysis. (rethinking) is it really duplication fault? replot independent
2. Discus why the end fault rate for the Mnist dataset is not as significant as predicted.
3. Dscus why the second layer is the most sensitive (tanh)
4. Fig 4 log x axis
5. why far away, add discussion 

Explain FPGAHammer work,
Fig 1 change, simplified 
Fig 6, e.g. how 100 faults, e,g, pulse width
what is a DSP slice add usage of DSP in DNN accelerator
how many slices on FPGA, can be configured to do
according to our empirical h

% 1. Describe the structure and components of the victim accelerator
%     a. loop structure is popular and is highly extendable e.g. DPU i.e. why we chose loop structure
%     b.  what is a DSP slice, why it is used in  DNN accelerators
% 2. Attack procedure
%     a. victim monitoring: execution analysis (TDC track)
%     b. attack guiding: identify the target layer
%     c. launch and tune the attack
%         1) we assume the adversary and query and obtain the result of victime MLaaS, which allows us to tune the intensity of the attack and find the more vulnerable layers
% Hence, our attack are mainly composed of two building blocks, victim monitoring and fault injection. We will introduce them in the following subsections.

\subsection{Attack Overview}
\subsubsection{The Victim}
In his work, we targeted the state-of-the-art DNN FPGA accelerator engine like Xilinx DPU and Apache DVM VTA. When given different instruction/opcode, these compute engines can compute multiple types of neural network layers like convolution layer, pooling layer, and fully connected layer. They also have parallel high-performance processing engines to handle the computation. These engines are typically implemented using digital signal processing (DSP) slices, which are dedicate hardware units on modern FPGAs that can accelerate a wide range of applications. In DNN accelerators, DSPs are mainly utilized to speed up multiplications and additions. More specifically, we chose an open-source DNN accelerate engine \cite{yolov2github} and trained a LeNet-5 neural network with MNIST dataset.
\subsubsection{Attack Procedures}
Our attacks is consist of three steps. The first step to obtain the execution information of the victim. We achieved this by mobilizing the TDC-based delay sensor to gather the side channel information leakage. The details of this step is discussed in sub section \ref{subsec:TDC}.

The second step is analyzing the information gathered in the previous step. The adversary would need to inspect and waveform and identify the time interval of the execution of each layer. Then one could test which layer is more susceptible to the attack.  This step is explained in sub section \ref{sec:attacking_scheduler}

The last step is launching the attack using power glitch fault injection. In sub section \ref{subsec:power_glitch} we described our fault injection capability and analyzed the fault characteristics.


==> Achieve/preliminary.tex <==
\section{DeepStike Attack}
% add overview here
\noindent
In this section, we evaluate the preliminary fault-injection results of the adversary before launching a full attack on DNN application. More specifically, we target the DSP slices where the majority of the computation happens.
%\subsection{Design of the voltage glitch circuit}
%Discuss possible designs of the attacking circuit. Argue the choice of ROs.
\subsection{Attack Overview}



\subsection{Power glitch Fault injection}
\subsubsection{Design of the power-plundering circuit}
%%\vspace{-0.5em}
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.5\linewidth]{FIG/FIG_PPC_ROL.pdf}
    \caption{A controllable and avoid DRC warning power-plundering cell design scheme that can be leveraged to construct malicious power-plundering circuit on FPGA.}
    \label{Fig:PW_circuit}
    %%%\vspace{-1.5em}
\end{figure}
%\noindent Design specific power-plundering circuits follow the virtual block. \\
%\textbf{Note:} The Ultrascale+ family has 8 LUTs in one logic slice. And the Ultrascale family only has 4 LUTs in one logic slice.
To achieve the power attack, the attacker would need to build a controllable and effective power-plundering circuit. When the circuit is enabled for a short period (e.g., a few clock cycles), it draws a significant amount of power, which create a voltage drop in the PDN. The voltage drop increase the signal propagation time in FPGA components that share the same PDN, which induce timing violations and potential faults.\cite{Krautter_Gnad_Tahoori_2018}

Previous work mainly utilized LUT based combination loops to implement the power-plundering circuit.  \cite{la2020fpgadefender,provelengios2020power} Those circuits are effective, but they lead to  design rule checking (DRC) warnings. A design with these warnings is not allowed to be deployed on the common cloud FPGA servers.\cite{8730895}

We develop a power-plundering circuit design that can pass the DRC check by inserting data latches in the combination loop. 

Fig. \ref{Fig:PW_circuit} describes our basic power-plundering circuit cell, which utilizes a two output look-up table ($LUT6\_2$) with two latch registers (LDCE). We set the $I5$ as $1'b1$ to activate two separate outputs, $O6$ and $O5$, and each of them connects with an LDCE. Compared with the combination loop design scheme, this method increases the loop's length and resistance. Not only can this design pass the DRC check, according to our experiment, it is more efficient as well. The advantage of this cell is that it has two self-oscillating loops for each LUT. It can reduce the number of LUT required to launch the attack. An adversarial multi-tenant FPGA tenant can apply a large number of such power-plundering cells, and use the same \textit{Enable} signal to control them. While the attacker activates this circuit at a designed moment, the specific timing violation will impact the executing DNN application.

\begin{figure*}[tb!]
    \centering
    \includegraphics[width=0.7\linewidth]{FIG/FIG_TDC_structure.pdf}
    \caption{The schematic of the FPGA TDC-based delay-sensor, and open-source YOLOv2 layer 7 to 9 power fluctuation tracing waveform.}
    \label{Fig:TDC_sch}
    % \vspace{-1.5em}
\end{figure*}
\subsubsection{Characteristics of the fault}\label{sec:DSP}
% here, describe what is DSP how it is used 5 sentences
To increase the performance of the DNN accelerators, designers often adopt a technique called double data rate, where the operating frequency of the DSP slices are twice of the frequency of the other components.\cite{pg338} This design choice makes the DSP slices more vulnerable to the power glitch attack because it have tighter timing constraints. According to our experiments, even if the DSP slices are not running at double frequency, they are sill vulnerable to our attack.

We designed experiments to observe the glitch induced faults in DSP slices. The DSP slices are configured to pre-add two inputs and multiply with the other input, which is the configuration for convolution computation \footnote{The fully connected layer are usually calculated in these configurations as well because they could be treated as special case of convolution}. Since the DSP slices does not have a result ready signal, we first designed a circuit that fetched the result of the DSPs after five clock cycles. This circuit works correctly and the timing analysis of the FPGA mapping tool does not complaint about violations of timing constraints.

For the first experiment we tested bare DSP slices operating at 400 MHz\footnote{The frequency is not high because it is twice of the main frequency due to the double data rate technique.}. We fed the DSP slices 1000 randomly generated inputs and launch the power-plundering circuit for one clock cycle at the same time we enabled the DSP slices. When utilizing 16,000 power-plundering cells, we can achieve nearly 100\% fault injection rate, i.e., nearly all of the computation results are incorrect. 

In the second experiment, we added input and output buffer registers that operate at half the frequency of the DSP to simulate the double data rate technique. We applied the same attack configuration as the first experiment's. The fault injection rate fell to around 60\%.

Although the input and output buffer reduce the fault injection rate, it does not affect the fault characteristics. We observed two type of faults. The first one we name as duplication fault, where the DSP output is the correct result of the previous input. In this case, the DSP computation simply takes longer to complete and cannot produce the correct result in time. The other type is random faults, where the faulty output does not have obvious patterns.

In Fig. \ref{Fig:DSP_exp}, we demonstrated both types of faults. The x axis is the number of power plundering cells, the y axis the number of faults of each type divided by the total number of experiments. DSP slice one and zero are on the same physical tile, while DSP two is on another physical tile. We can observer that different DSP slices have different fault characteristics. Some mainly random faults while others have nearly the same amount of random faults and duplication fault, which makes it hard to precisely control the faults. Moreover, the fault rate grows nearly linearly with the number of power-plundering cells. When we use 24,000 cells, the total fault rate is nearly 100\%.\footnote{total fault rate is the sum of duplication fault rate and random fault rate. When launching the real attack, we would need less power-plundering cells because the victim consumes power, which reduces the voltage of the PDN. } Hence, we can control the fault injection intensity by adjusting the number of power-plundering cells.
%%%%\vspace{-0.5em}
% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=1\linewidth]{FIG/FIG_DSP_exp.pdf}
%     \caption{Duplication fault  rate and random fault  rate of double data rate DSP slices with different number of power-plundering cells.\textcolor{red}{why we have two types of faults in this paper}\textcolor{blue}{we observed two types of faults. We are re-plotting this figure to make it more clear}} 
%     \label{Fig:DSP_exp}
%     % %%%\vspace{-1.5em}
% \end{figure}

\begin{figure}[tb!]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{FIG/FIG_DSP_Ex_xilinx_setup.pdf}
        \caption{The Xilinx FPGA (XC7Z020) layout for the DSP fault injection test.}
        \label{Fig:layout_DSP}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{FIG/FIG_DSP_Ex_xilinx_setup.pdf}
        \caption{The Intel FPGA (XXXX) layout for the DSP fault injection test.}
        \label{Fig:layout_DSP}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{FIG/FIG_DSP_exp.pdf}
        \caption{Xilinx FPGA: Duplication fault  rate and random fault rate of double data rate DSP slices with different number of power-plundering cells.}
        \label{Fig:DSP_result}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{FIG/FIG_DSP_exp.pdf}
        \caption{Intel FPGA: Duplication fault  rate and random fault rate of double data rate DSP slices with different number of power-plundering cells.}
        \label{Fig:DSP_result}
    \end{subfigure}
    \caption{DSP fault injection test configurations and results on both Xilinx and Intel FPGA.}
\label{Fig:DSP_exp}
\end{figure}








%\noindent\textcolor{red}{Ex.1.1 Result(Cheng's experimental result in this section.)}\\
%Describe the fault characteristics in DSP slices. Provide fault metrics.

% \subsection{Fault propagation in convectional kernel}
% % \noindent\textcolor{red}{Ex.1.2 Result(Cheng's experimental result in this section.)}\\

% We have shown the faults injected in the DSP are partially dependent on the input. Hence, we would need a real model to quantitatively measure the fault propagation in the convolution kernel.  In this section, we explore how the faults in the DSP units are accumulated in the fist layer.

% %%\vspace{-0.5em}
% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=1\linewidth]{FIG/FIG_MNIST_Case_study.pdf}
%     \caption{Fault propagation in convectional kernel}
%     \label{Fig:DPU_Fault}
%     % %%\vspace{-1.5em}
% \end{figure}

% \subsection{Evaluation of the vulnerability of DNN accelerator kernels}
% Random attack on DNN convolutional kernel:\\
% (1) What is the attack configuration? For voltage glitch attack, in what convolutional kernel computing stage can we activate the attack? and how long is the attacking time?  \\
% (2) What happens while we place the attack, report the error rate and the error methodology. \\
% (3) Introduce our attacking performance metrics and visible results. 


% \section{Attacking the DNN application on multi-tenant FPGA}

% \noindent \textbf{attacking steps:}\\ 
\subsection{TDC based Victim monitor}\label{sec:atk_step}
% here, describe the specific victim, justify generality in the end
% \begin{figure*}[tb!]
%     \centering
%     \includegraphics[width=0.7\linewidth]{FIG/FIG_TDC_structure.pdf}
%     \caption{The schematic of the FPGA TDC-based delay-sensor, and open-source YOLOv2 layer 7 to 9 power fluctuation tracing waveform.}
%     \label{Fig:TDC_sch}
%     % \vspace{-1.5em}
% \end{figure*}


\subsubsection{TDC design}


%An example FPGA TDC implementation is shown in Fig. \ref{Fig:TDC_sch}, which is composed of two major components: delay-line and 


The proposed TDC-based delay-sensor shows in Fig. \ref{Fig:TDC_sch}. It can be seen that different activities have distinct voltage profiles. We denoted two main components: $DL_{LUT}$, a LUT-based delay-line, and $DL_{CARRY}$, a carry-chain based delay-line. The length of $DL_{LUT}$ determines the sensitivity of this delay-sensor, and the $DL_{CARRY}$ can scale the output range. The phase difference $\theta$ of two clock signals, driving clock and sampling clock, can calibrate the output. As we show in figure \ref{Fig:TDC_sch}, the ideal output method, a consecutive “1” output starts at the least significant bit (LSB) output, and the rest output are all zeros. We count the number of consecutive “1” as the output to represent the internal components’ propagation delay status, and we set the unit as “bin” \cite{zick2013sensing}. While the power attack applies to the corresponding FPGA, the bin will reduce. The driving clock frequency ($F_{dr}$) and the length of $DL_{LUT}$ ($L_{LUT} $)and $DL_{CARRY}$ ($L_{CARRY}$) should be carefully designed to avoid counting errors. In this paper, we set $F_{dr} = 200MHz$, $L_{LUT} = 4$,and $L_{CARRY} = 128$. 

%\noindent
%(1) Tracing the DNN application by a TDC sensor and collecting the target DNN application's execution tracing diagram.\\ 
%(2) Analyzing the DNN tracing diagram and exploring it with DNN knowledge from open-source Model Zoo to decide the attacking object and extract them as critical parameters for our attacking guide machine\\ 
%(3) Using our proposed attacking guide machine to place an attack on different DNN layers and achieve our results to reduce the target DNN model's prediction accuracy.

Our preliminary study proves that the power glitch attack can impact the convolution kernel based on DSP components. In other words, the proposed power glitch attack can impact all components under the same power supply VCCINT, and the attacker can place the attack on all acceleration layers implemented on FPGA in a DNN application. Compared with \cite{frakin2020deep}, the focus of our paper is 
the on-chip power side-channel leakage on the cloud-FPGA. An adversary tenant can gather this leakage and place attacks on the target DNN layer effectively. 

In a practical scenario, the attacker may not have enough knowledge about the model parameters. 
Therefore, the primary challenge of this task is to trace the target DNN application implementation. A TDC-based delay-sensor shown in section \ref{sec:TDC} is useful, which can measure the on-chip side-channel leakage while the DNN application is executing. Figure \ref{Fig:TDC_sch}(a) provides a tracing example on an FPGA YOLOv2 accelerator \cite{yolov2github}, which implements the layer 7 to the layer 9. The layer 7 is a max-pooling layer; the layer 8 is a convolution layer with a $3 \times 3$ kernel. And layer 9 is a  convolution layer with a $1 \times 1$ kernel. The TDC-based delay-sensor consists of a 128-bits carry-chain and several LUTs. We notice clear stalls between different layer implementations, and the power fluctuation in the execution of the convolution layer is more massive than that of the max-pooling layer. We can pick up several register outputs from the original 128-bits carry-chain outputs with a careful analysis and design to optimize them as down-sampling outputs. As figure \ref{Fig:TDC_sch}(b) shows, the clear stalls and various power fluctuation ranges provide enough information to identify different execution periods among different layers. Associated with some public information, such as Model Zoo \cite{modelzoo}, an adversary can infer the layer type and know the network architecture. Those analyses and discussions may make the attack more efficient, but in our threat model, we consider that the attacker can only gather on-chip side-channel leakage. After the analysis and measurement steps, an adversary can utilize the optimized down-sampling TDC-based delay-sensor to build an attacking scheduler. This scheduler can place several attacks on different layers or in different application execution periods. We will introduce the attacking scheduler’s structure in section \ref{sec:attacking_scheduler} and demonstrate a case in section \ref{sec:case_study}. 



%Our preliminary study proves that the power glitch attack can impact the convolution kernel based on DSP components. 
%% Paper \cite{frakin2020deep} introduces an adversarial weight duplication (AWD) hardware attack on the FPGA BRAM at the weight transmission process. 
%In other words, the proposed power glitch attack can impact all components under the same power supply VCCINT, which means that in the DNN application, the attacker can place the attack on all acceleration layers implemented on FPGA. Compared with \cite{frakin2020deep}, our paper focuses on the multi-tenant FPGA power on-chip side-channel leakage. An adversary tenant can gather this leakage and place attacks on the target DNN layer effectively. In a practical scenario, the attacker may not have access to the prediction output and have enough knowledge about the model parameters. Therefore the primary challenge of this task is to trace the target DNN application implementation. A TDC-based delay-sensor shows in section \ref{sec:TDC} is useful, which can measure the on-chip side-channel leakage while the DNN application is executing. Figure \ref{Fig:YOLO_Trace}(a) provides a tracing example on an FPGA YOLOv2 accelerator \cite{yolov2github}, which implements layer 7 to layer 9. Layer 7 is a max-pooling layer; layer 8 is a convolution layer with $3 \times 3$ kernel. And layer 9 is a  convolution layer with $1 \times 1$ kernel. The TDC-based delay-sensor consists of a 128-bits carry-chain and several LUTs. We notice clear stalls between different layer implementations, and the convolution layer can achieve more massive power fluctuation rather than max-pooling layer execution. We can pick up several register outputs from the original 128-bits carry-chain outputs with careful analysis and design to optimize them as down-sampling outputs. As figure \ref{Fig:YOLO_Trace}(b) shows, the clear stalls and various power fluctuation ranges provide enough information to identify the difference between layers and the execution period. Associate with some public information, such as Model Zoo \cite{modelzoo}, an adversary can infer the layer type and know the network architecture. Those analyses and discussions may make the attack more efficient, but in our threat model, we consider that the attacker can only gather on-chip side-channel leakage. After the analysis and measurement steps, an adversary can utilize the optimized down-sampling TDC-based delay-sensor to build an attacking scheduler. This schedular can place several random attacks on different layers or application execution period. We will introduce the attacking scheduler’s structure in section \ref{sec:attacking_scheduler} and demonstrate a case in section \ref{sec:case_study}. 


% % %%\vspace{-0.5em}
% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=1\linewidth]{FIG/FIG_TDC_Trace_7_9.pdf}
%     \caption{Open source YOLOv2 layer 7 to 9 power fluctuation measured by TDC-based delay-sensor.}
%     \label{Fig:YOLO_Trace}
%     % %%\vspace{-1.5em}
% \end{figure}


==> TEXT/Sec.0_abstract.tex <==
%The deployment of the Deep Learning Neural Network (DNN) applications raise researchers’ interest in the hardware accelerator. As a result, field-programmable gate arrays (FPGAs) become the hot device in developing the acceleration platforms. However, the high upfront investment suffers the individual researcher, developer, and emerging enterprises. 
%To solve this problem, researchers explored the FPGA virtualization and on-demand hypervisor-level system to enable the feature that multiple independent tenants can access and share the resource in the same FPGA device. Such a multi-tenant FPGA setup for the DNN accelerator creates a unique attack surface. The malicious tenants gather the power leakages to threaten the DNN interference task. This paper proposes the DeepStrike attack, which utilizes the time-to-digit converter (TDC) as the on-chip delay-sensor to measure the on-chip side-channel power leakages. After the pre-measurement, our specific designed power glitch attacking scheduler can guide and place a particular number of random attacks to impact the target DNN interference circuit’s acceleration kernels. We also explore the DNN’s convolution kernel’s timing fault properties on the FPGA’s DSP components and provide a study case to demonstrate our proposed attacking process. 
%%%%%%%%%%%%%%%%% DAC 2021 submission version (100 words) %%%%%%%%%%%%%%%%%
\if false
Field-programmable gate arrays (FPGAs) virtualization enables multiple users to share FPGA chip on the cloud, which significantly improves the efficiency of compute-intensive applications like Deep Neural Network (DNN), but also brings new security concerns. This work focuses on the security of DNN accelerator on cloud-FPGA and makes two contributions: 1) characterizing the vulnerabilities of different DNN layers against fault injection attack, and 2) presenting \ourtit, a remotely-guided fault injection attack targeting the most vulnerable DNN layer. To locate the critical timing for fault injection, i.e., during the execution of the most vulnerable DNN layers, \ourtit ~leverages the side-channel leakage of delay-sensors based on time-to-digital converter (TDC). Experimental results demonstrate that \ourtit can successfully inject timing violations in the DNN accelerator implemented on FPGA DSP components. The timing violations will delay or corrupt each DSP's desired outputs to create junk data, which mislead the next layer calculation or directly apply to the prediction outputs.
\fi
\if false
As Field-programmable gate arrays (FPGAs) are widely adopted in clouds to accelerate Deep Neural Networks, such virtualization environments have posed many new security issues. This work investigates the integrity of DNN FPGA accelerators in clouds. It proposes \texttt{DeepStrike}, a remotely-guided attack based on voltage glitching fault injections targeting DNN execution.  We characterize the vulnerabilities of different DNN layers against fault injections on FPGAs, and leverage time-to-digital converter (TDC) sensors to precisely control the timing of fault injections. Experimental results show that our proposed attack can successfully disrupt the FPGA DSP kernel and result in misclassifications of a victim CNN model on MNIST datasets. 
\fi
As Field-programmable gate arrays (FPGAs) are widely adopted in clouds to accelerate Deep Neural Networks (DNN), such virtualization environments have posed many new security issues. This work investigates the integrity of DNN FPGA accelerators in clouds. It proposes DeepStrike, a remotely-guided attack based on power glitching fault injections targeting DNN execution.  We characterize the vulnerabilities of different DNN layers against fault injections on FPGAs and leverage time-to-digital converter (TDC) sensors to precisely control the timing of fault injections. Experimental results show that our proposed attack can successfully disrupt the FPGA DSP kernel and misclassify the target victim DNN application. 

%\textcolor{red}{add some details of the experiment, no worries about the word count now.}. %Furthermore, we explore the fault characterization of the convolution kernel accelerator deployed on the FPGA DSP components and provide a study case to demonstrate our proposed attacking process, which can successfully reduce the inference accuracy.




%Field-programmable gate arrays (FPGAs) enable versatile and efficient Deep Neural Network (DNN) accelerators. FPGAs virtualization effectively utilizes an FPGA chip by allowing multiple users to configure it on the cloud partially. Such a multi-tenant FPGAs setup creates a new attack surface. This work proposes the \texttt{DeepStrike} attack, where the colocating adversary employs the time-to-digit converter (TDC) to guide the carefully crafted remote power glitch attack. We explore the fault characterization of DNN accelerators with DSP slices and provide a case study to demonstrate our proposed attack, which can successfully reduce the inference accuracy.


